Separatrices: the crux of reconnection

Reconnection is one of the key processes in astrophysical and laboratory plasmas: it is the opposite of a dynamo. Looking at energy, a dynamo transforms kinetic energy in magnetic energy while reconnection takes magnetic energy and returns is to its kinetic form. Most plasma processes at their core involve first storing magnetic energy accumulated over time and then releasing it suddenly. We focus here on this release. A key concept in analysing reconnection is that of the separatrix, a surface (line in 2D) that separates the fresh unperturbed plasma embedded in magnetic field lines not yet reconnected with the hotter exhaust embedded in reconnected field lines. In kinetic physics, the separatrices become a layer where many key processes develop. We present here new results relative to the processes at the separatrices that regulate the plasma flow, the energisation of the species, the electromagnetic fields and the instabilities developing at the separatrices.

==> instabilities.tex <==

\section{Separatrices as loci of instabilities}
\label{sect-instabilities}
Observing closely the electric field strucutures near the separatratrices (see the insets in Fig~\ref{hall_signatures}-\ref{other_signatures}), instabilities can be observed in the parallel and perpendicular components. 

{\color{red} Description of the types of instabilities seen in our previous work and their origin. Stefano and Andrey lead writing

Andrey: 

Descriuption of electron holes and their original

Description of electromagnetic instabilities and their origin

Stefano:

Extension to 3D 
}
